Branching via Cutting Plane Selection: Improving Hybrid Branching

Cutting planes and branching are two of the most important algorithms for solving mixed-integer linear programs. For both algorithms, disjunctions play an important role, being used both as branching candidates and as the foundation for some cutting planes. We relate branching decisions and cutting planes to each other through the underlying disjunctions that they are based on, with a focus on Gomory mixed-integer cuts and their corresponding split disjunctions. We show that selecting branching decisions based on quality measures of Gomory mixed-integer cuts leads to relatively small branch-and-bound trees, and that the result improves when using cuts that more accurately represent the branching decisions. Finally, we show how the history of previously computed Gomory mixed-integer cuts can be used to improve the performance of the state-of-the-art hybrid branching rule of SCIP. Our results show a 4% decrease in solve time, and an 8% decrease in number of nodes over affected instances of MIPLIB 2017.

==> todo.tex <==
% Add counter for how frequentlz instances arrive at GMI tiebreaker (how many times does this actually affect the rbanching decision)
% Add summary of hybrid branching. Put this in the appendix or something. 
% Experiments: Print out amount of times GMI cut branching resulted in a new best scoring decision. 
% - In the case of a different decision, how frequent was there formerly a tie. (How frequently do we get a tie still?) Do this both over the search tree and the root node
% Experiments: At the root node, over all branching candidates, over all hybrid branching criteria, do we have values intiailised? Get the ratio of how many times GMI is initialised compared to all the other measures. 
